Max-Consensus Over Fading Wireless Channels

The topic of this paper is achieving finite-time max-consensus in a multi-agent system that communicates over a fading wireless channel and exploits its interference property. This phenomenon corrupts the desired information when data is transmitted synchronously. In fact, each transmitted signal is attenuated by an unknown and time-varying factor (fading coefficient), then, by interference, all such attenuated signals are summed up at a receiver. Rather than combatting interference, we design a communication system that exploits it. Our strategy yields a more efficient usage of wireless resources compared to other algorithms. By simultaneously accessing this communication system, each agent obtains a weighted average of the neighbouring agents' information states. With this piece of information at hand and with a switching consensus protocol employing broadcast authorisations for agents, max-consensus can be achieved within a finite number of iterations.

==> communication_system.tex <==
\subsection{{Wireless Multiple Access Channel}}
\label{sec:wirelessMAC}
% The broadcast property of radio signals in a multi-agent communication system is often utilized for transmitting signals simultaneously to all listening neighbors. However, in general, interference is avoided, and each tranmission is restricted to orthogonal resources. Even in a fully-connected networks this strategy will require at least $N$ independent uses of communication resources for sharing of information among all the agents. However, in most Wireless Sensor Networks (WSN) applications, the functional computation at the receiver have implicit similarities to the channel's input and output structure. In such cases, a joint source-channel communication approach is superior than separation-based approaches \cite{Gastpar2006}. In this work, we harness the interference property of the WSN for solving max-consensus problems.

%We model the Linear Time-Variant (LTV) wireless channel as flat-fading and narrow-band. This assumption leads to a simplified \textit{single-tap} channel model, where channel is assumed to be constant for a time period (coherence time) much greater than the symbol duration. 
Let $\mathcal{T}=\{1,\dots,N\}$
be a set of transmitters.
Let, $\forall j\in\mathcal{T}$, 
$\omega_j : \mathbb{N} \mapsto \mathbb{C}$
be the transmitted signal,
at a given iteration,
by agent $j$. 
The signal received in response to a 
synchronized transmission by all agents in $\mathcal{T}$
can be described as a 
superposition of 
their transmitted signals.
This system is called 
\textit{Wireless Multiple Access Channel (WMAC)}.

\begin{definition}[Wireless Multiple Access Channel (WMAC)]
	\label{def:MAC}
	The multiple access channel 
	between $N$ synchronized transmitters and a receiver
	is a map $\mathcal{W}: \mathbb{C}^N \mapsto \mathbb{C}$
	given by,
	\begin{equation}
		\label{eq:WMAC}
		{
	%	\mathcal{W}: \big( \omega_1(k),\dots, 
	%	\omega_N(k) \big) \mapsto 
	%	\sum_{j=1}^N \xi_j(k)\, \omega_j(k) + \eta(k)

	\forall k\in\mathbb{N}, \\
		\mathcal{W} \big( \omega_1(k),\dots, 
		\omega_N(k) \big) :=
		\sum_{j=1}^N \xi_j(k)\, \omega_j(k) + \eta(k),
		}
	\end{equation}
	where, 
	$\forall k\in\mathbb{N}$,
	$\forall j\in\mathcal{T}$,
	$\omega_j(k) \in \mathbb{C}$ is the 
	signal broadcast by agent 
	$j \in \mathcal{T}$,
	with $|\omega_j(k)|^2 \leq P_{\max}$, 
	where $P_{\max} > 0$ is the maximum transmit power; 
	$\forall j\in\mathcal{T}$,
	$\xi_j: \mathbb{N} \mapsto \mathbb{C}$ is the 
	Channel Impulse Response (CIR) 
	between the transmitter $j\in\mathcal{T}$ 
	and the receiver.
	$\eta: \mathbb{N} \mapsto \mathbb{C}$ is the Additive White Gaussian Noise (AWGN).
\end{definition}

In \cite{goldenbaum2013robust},
authors considered an \textit{ideal} WMAC channel 
where 
$\forall k \in \mathbb{N}$,
$\forall j \in \mathcal{T}$, 
$\xi_j(k) = 1$ and $\eta(k) = 0$. 
In this ideal case, the channel output is a plain sum of 
channel inputs, i.e. 
$\mathcal{W}_{\text{ideal}}: \big( \omega_1(k),\dots, \omega_N(k) \big) \mapsto \sum_{j=1}^N \omega_j(k)$. 
However, in practice, both channel coefficients $\xi_j(k)$ and the AWGN $\eta(k)$ corrupt the output at the receiver. 
Hence, in this work, 
algorithms that consider a
practical WMAC, as defined in (\ref{eq:WMAC}),
will be considered.

In the spirit of \cite{molinari2018exploiting},
the consensus protocol of Section \ref{sec:asyCons}
will require,
at each receiver $l\in\mathcal{N}$,
an input $u_l$ that has to hold
some conditions:
first, $\forall l\in\mathcal{N}$,
$u_l\in\mathbb{R}$;
second, $\forall l\in\mathcal{N}$,
$u_l\in\mathcal{C}(\{x_j\mid j\in\mathcal{T} \})$.
The following communication
system will be designed
in order to guarantee
these two conditions.

\section{{Communication system design}}
\label{sec:commsys}
%The WMAC creates a unique mapping
%between its inputs and output, 
%while the nomographic representation provides 
%a framework to harness this mapping. 
%In this section, 
%a communication system 
%implementing
%this mapping,
%while holding practical considerations,
%is designed.
Every agent is equipped with a full-duplex radio and signal-processing capabilities to facilitate simultaneous transmission and reception of signals \cite{choi2010achieving}. In practice, perfect synchronization between multiple transmitters and receivers is extremely difficult. Therefore, a coarse synchronization scheme 
using analog transmissions, as described in \cite[p.87-94]{goldenbaum2014computation},
is employed. 
%A block diagram of
%the communication system 
%that will be
%presented throughout 
%this section
%is shown 
%in Figure \ref{fig:commsys}.

%This scheme is based on the assumption that at least $M \in \mathbb{N}$ symbols can be transmitted within a duration $\Delta t$ less that the coherence time period $T_c$ of the channel, during which the channel remains constant (in the mean-square sense) \cite[p.19]{Matz2011}.

%\begin{equation}
%	\mathbb{E}_{\xi \sim p(\xi)}\{\lvert \xi_{ij}(k + m) - \xi_{ij}(k)\rvert^2\} \approx 0
%\end{equation}
%where $\mathbb{E}_{p}\{\cdot\}$ stands for expectation over the probability distribution $p$, $\xi_{ij}(k)$ is the channel fading coefficient between $i$ and $j$ at time instant $k$, and $0 \leq m \leq M$ is the discrete time-steps for which channel remains constant, with $M \leq \frac{T_c}{T_s}$ and $T_s$ as sampling time. By repeating the transmission $M$ times, distortions caused by mismatching phases and additive white Gaussian noise (AWGN) can be averaged out.

%The agents are grouped into $L$ overlapping clusters with an agent $l \in \mathcal{L}$ as the cluster-head, and all its neighboring agents $\mathcal{N}_l$ as members of the cluster, that is, $\mathcal{C}_l := \{l  \cup \mathcal{N}_l\}$. Clusters are chosen in such as way that each member $j \in \mathcal{N}$ must belong to at least one of the clusters, and is connected to every other members (strongly-connected network) through some sequence of overlapping clusters. The role of the cluster-head is to compute the \emph{sum} of information transmitted by neighboring agents, and broadcast it back along with its own information. In this way, every agent can obtain a function of information states of all agents in the cluster (equation (\ref{eq:generalConsProt})) in just one communication cycle.

%The desired function is represented by its nomographic form, as in equation (\ref{eq:nomo}). 

% In order to have real input and output of the system, we employ a two step communication protocol that allows superposition of the amplitudes of signals, while canceling the phases. A block diagram of the communication system is presented in Figure \ref{fig:WMAC}.

\begin{figure}[t!]
	\centering
	\resizebox{\columnwidth}{!}{
		\begin{tikzpicture}
		\tikzset{bigarrow/.style={decoration={markings,mark=at position 1 with {\arrow[scale=1.5,>=stealth]{>}}},postaction={decorate}}}
		\tikzset{rbox/.style={draw, rectangle, minimum size=8mm}}
		\tikzset{antenna/.style={draw, regular polygon, regular polygon sides=3, fill=black, inner sep=0.5mm, outer sep=0mm, rotate=180}}
		
		% transmitter
		\node (input) at (3,0) {};
		\node (input2) at (4.5, -2) {};
	%	\node[rbox] (tr1) at (2,0) {$\phi_j(\cdot)$};
		\node[rbox] (tr2) at (4.5,0) {$\sqrt{\Phi(\cdot)}$};
		% \node[rbox] (tr3) at (6,0) {$\sqrt{\cdot}$};
		\node[draw, circle, inner sep=0mm, outer sep=0mm, minimum size=2mm] (cross) at (6,0) {$\times$};
		\node (phase) at (6,1) {$\pmb{\nu}_j$};
		\node[draw, circle, inner sep=0mm, outer sep=0mm, minimum size=2mm] (cross2) at (6,-2) {$\times$};
		\node (phase2) at (6,-1) {$\pmb{\nu}'_j$};
		
		\node[inner sep=0mm, outer sep=0mm] (tr6) at (7,0) {};
		\node[antenna] (tr7) at (7,0.5) {};
		\node[anchor=south] (tr7) at (7,0.5) {$j$};
		\node[inner sep=0mm, outer sep=0mm] (tr62) at (7,-2) {};
		\node[antenna] (tr72) at (7,-1.5) {};
		\node[anchor=south] (tr72) at (7,-1.5) {$j$};
		
		%channel
		\node[draw, circle, dotted, inner sep=1mm, outer sep=0mm, minimum size=5mm] (block2) at (8,0.2) {$\xi_{jl}$};
		\node[draw, circle, dotted, inner sep=1mm, outer sep=0mm, minimum size=5mm] (block3) at (8,-1.7) {$\xi_{jl}$};
		
		%receiver
		\node[inner sep=0mm, outer sep=0mm] (rx3) at (8.7,0) {};
		\node[antenna] (rx4) at (8.7,0.5) {};
		\node[anchor=south] (rx4) at (8.7,0.5) {$l$};
		\node[rbox] (rxG) at (9.8,0) {$\Gamma(\cdot)$};
		\node[rbox] (rx5) at (11.5,0) {$\Psi(\cdot)$};
		\node[inner sep=0mm, outer sep=0mm] (rx32) at (8.7,-2) {};
		\node[antenna] (rx42) at (8.7,-1.5) {};
		\node[anchor=south] (rx42) at (8.7,-1.5) {$l$};
		\node[rbox] (rxG2) at (11.5,-2) {$\Gamma(\cdot)$};
		
		\node[rbox] (rx43) at (12.5,-1) {$\frac{\gamma_l}{\gamma'_l}$};
		
	%	\node[rbox] (rx6) at (16,-1) {$\psi_l(\cdot)$};
		\node (rx7) at (13.8,-1) {};
		\node (rx72) at (13.8,-2) {};
		
		\draw[dashed] (7.4, 1.5) node[anchor=south east] {$j = 1, \dots, |{N}_l|$} rectangle (3, -2.5);
		
		\draw[bigarrow] (input) -- node[anchor=south] {$x_j$} (tr2);
	%	\draw[bigarrow] (tr1) -- node[anchor=south] {$\kappa_j$} (tr2);
		\draw[bigarrow] (tr2) -- node[anchor=south] {$\mu_j$} (cross);
		\draw[bigarrow] (phase) -- (cross);
		\draw[bigarrow] (cross) -- node[anchor=south] {$\pmb{\omega}_j$} (tr6);
		\draw[-] (tr6) -- (tr7);
		
		\draw[bigarrow] (input2) -- node[anchor=south east, pos=0.8] {$\mu'_j = 1$} (cross2);
		\draw[bigarrow] (phase2) -- (cross2);
		\draw[bigarrow] (cross2) -- node[anchor=south] {$\pmb{\omega}'_j$} (tr62);
		\draw[-] (tr62) -- (tr72);
		
		\draw[-] (rx3) -- (rx4);
		\draw[-] (rx3) -- node[anchor=south]  {$r_l$} (rxG);
		\draw[bigarrow] (rxG) -- (rx5);
		\draw[bigarrow] (rxG2.north) -- node[anchor=west] {$\gamma'_l$} (rx5.south);
		\draw[bigarrow] (rx5) -| node[anchor=south west, pos=0.3] {$\gamma_l$} (rx43);
		\draw[-] (rx32) -- (rx42);
		\draw[bigarrow] (rx32) -- node[anchor=south]  {$r_l'$}  (rxG2);
		\draw[bigarrow] (rxG2) -| node[anchor=north west, pos=0.3] {$\gamma'_l$} (rx43);
	%	\draw[bigarrow] (rx43) -- (rx6);
		\draw[bigarrow] (rx43) -- node[anchor=south] {$\hat{f}_l$} (rx7);
		\end{tikzpicture}
	}
	\caption{Detailed design of the communication system.}
	\label{fig:commsys}
\end{figure}

% New part by Fabio
At every iteration $k \in\mathbb{N}$
of the consensus protocol,
the communication system, described in Figure \ref{fig:commsys},
guarantees that the state informations are exchanged between
all the neighboring agents.
%In the remainder of this section,
%the communication system of Figure \ref{fig:commsys} 
%is designed;
%it guarantees that agents exchange
%information at an arbitrary iteration $k\in\mathbb{N}$
%of their consensus protocol. 
For the ease of exposition, 
the consensus protocols' iteration index $k$
is omitted from variables that 
remains constant during the execution
of the communication protocol.



%Assume that the system is in the $k$-th iteration of the consensus protocol. Each iteration requires exchange of information among neighboring agents, which is achieved by the communication system in $M$ time-steps. In the following discussion, we ignore the iteration counter $k$ in the expressions. It must be clear that the state information transmitted by agents corresponds to the $k$th iteration, and after $M$ time-steps, the system will complete exchange of information and reach the iteration $k+1$.

\subsection{Channel characteristics and assumptions}
The channel fading coefficient 
%$\xi: \mathbb{R} \times \mathbb{R} \mapsto \mathbb{C}$ 
is a 2D random process in time and frequency domains
(see \cite[Sec. 6.3]{Molisch2010}). 
The channel is assumed to be constant in frequency domain;
this assumption is valid in 
practice for stationary environments, 
and can be further ensured 
by using narrow-band signals, i.e. the bandwidth of the 
signal is much smaller that the carrier frequency. 
In what follows,
let,
$\forall i\in\mathcal{N}$
(receiver),
$\forall j\in \mathcal{T}$
(transmitter),
$\xi_{ji}:\mathbb{N}\mapsto\mathbb{C}$
be
the respective
fading coefficient.
It is assumed
to be distributed as a
complex
Gaussian random variable, i.e.,
$\forall i\in\mathcal{N}$,
$\forall j\in \mathcal{T}$,
$\xi_{ij}\sim\mathcal{C}\mathcal{N}(\bar{\xi}_{ij},\sigma_{\xi_{ij}}^2)$.
The channel is also assumed 
to be a
\textit{uncorrelated} between different users. 
this leads to major simplifications 
that any two distinct realizations 
of the channel will 
be uncorrelated, 
i.e., $\forall i,j,l \in \mathcal{N}$,
$i \neq j \neq l \implies\mathbb{E}\{ \xi_{ij} \xi^*_{il}\} = 0$. 
%and second, 
%the correlation function between 
%channel ensembles at two 
%different time instances 
%will be a function of the 
%time difference only; 
%i.e., $\forall j,l \in \mathcal{N}$,
%$\forall k,k' \in \mathbb{N},\ 
%\mathbb{E}[\xi_{ij}(k) \xi_{ij}^*(k')] = f(k-k')$. 

Another valid assumption in a stationary environment is of \textit{slow-fading}
(see \cite{Tse2012}). 
In this regime, the amplitude and phase changes 
(due to the channel) can be considered roughly constant over the coherence time period $T_c$, which is usually much greater than the symbol duration $T_s$,
i.e.
\begin{equation}
	\small
	\forall (i,j)\in\mathcal{A},\
	\forall m',m'' \in\{1,\dots,M\},\
	\xi_{ij}(m')
	\approx
	\xi_{ij}(m'')
	,
\end{equation}
where $M \leq \lfloor T_c/T_s \rfloor$.
The designed communication scheme is
based on the assumption that at least $M \in \mathbb{N}$ symbols can be transmitted within the coherence time period $T_c$ of the channel, during which the channel remains constant.

\subsection{Transmitter design}
%Agent $l \in \mathcal{N}$ 
%receives signals broadcast by 
%agents in $\mathcal{T}$. 
Each agent $j\in\mathcal{T}$ 
needs to transmit its
information state $x_j: \mathbb{N} \mapsto \mathrm{S}$ to its neighbor $l \in \mathcal{N}$.
In order to transmit this 
information over a 
power-constrained 
radio transmitter, 
a linear transformation 
$\Phi: \mathrm{S} \mapsto \mathrm{P}:= [P_{\min}, P_{\max}] \subset \mathbb{R}$
followed by square-root operator $\sqrt(\cdot)$
is applied. 
Transformation $\Phi$ can be designed with the knowledge of 
range of $\mathrm{S}$ and $\mathrm{P}$. 
Given $\alpha = \frac{P_{\max} - P_{\min}}{S_{\max} - S_{\min}} \in \mathbb{R}_{>0}$ and 
$\beta = P_{\min} - \alpha S_{\min}$, 
we have $\Phi(x_j) = \alpha x_j + \beta$ 
\footnote{$P_{\min}$ guarantees a high SNR regime.}.
The transformed information, given by $\mu_j := \sqrt{\Phi(x_j)}$ 
is modulated on the amplitude of a sequence of signals. 

%The receiving agent $l$ receives a linear weighted sum of transmitted signals, as given by equation (\ref{eq:WMAC}), and apply a post-processing function $\psi_l : \mathbb{R} \mapsto \mathrm{S}$ to obtain the nomographic representation. Notice that in a nomographic representation of a real-valued function, the pre- and post-processing functions are real valued. The radio signals, on the other hand, are complex. We present a communication system design that implements nomographic representation with real-valued input-output on the complex-valued WMAC (Fig. \ref{fig:commsys}).

For each transmitter
$j \in \mathcal{T}$,
a sequence of 
$M$ symbols,
grouped in vector
$\pmb{\nu}_j = [\nu_j(1), \dots, \nu_j(M)] \in \mathbb{C}^M$,
are independently generated. 
In what follows, 
$\forall j\in\mathcal{T}$,
$\forall m\in\{1,\dots,M\}$,
$\nu_j(m) = e^{\iota \theta_j(m)}$, 
where $\iota = \sqrt{-1}$,
and 
%$\forall m \in \{1,\dots,M\}$,
%$\forall j\in{N}_l$,
$\theta_j(m)$ is an i.i.d. random variable $\forall j \in \mathcal{T},\ \forall m \in \{1, \dots, M\}$ uniformly distributed on 
$[0, 2\pi)$. 
The sequence of 
symbols 
broadcast by each 
$j \in \mathcal{T}$
is,
then,
given by
\begin{equation}
%	\forall m \in \{1,\dots,M\}\\
	\pmb{\omega}_j := \mu_j \pmb{\nu}_j = \Big[ \mu_j e^{\iota \theta_j(1)}, \dots, \mu_j e^{\iota \theta_j(M)} \Big]\ \in \mathbb{C}^M.
\end{equation}

Another simultaneous transmission over an orthogonal 
channel is used to send a dummy pilot signal, i.e.,
$\forall j\in\mathcal{T}$,
$\mu'_j = 1$. 
This signal is influenced by the same channel 
$\xi_{jl}$, and, hence,
can be used by the receiver to estimate the sum of channel fading coefficients from all agents. 
A sequence of symbols $M$
for this signal is 
generated in the same way as above,
i.e.
\begin{equation}
	\pmb{\omega}'_j := \mu'_j \pmb{\nu}'_j = \Big[ e^{\iota \theta'_j(1)}, \dots, e^{\iota \theta'_j(M)} \Big]\ \in \mathbb{C}^M.
\end{equation}

\subsection{Receiver design}
By Definition \ref{def:MAC},
the vector resulting from
the superimposition
at the receiver $l\in\mathcal{N}$
of 
the broadcast sequences of $M$ symbols, $\pmb{r}_l\in\mathbb{C}^M$
is defined as
\begin{equation}
	\label{eq:rl}
	\pmb{r}_l := \left[ \sum_{j\in \mathcal{T}} \omega_j(m) \xi_{jl}(m) + \eta_l(m) \right]_{m=1}^M
	,
\end{equation}
where $\forall m\in\{1,\dots,M\}$,
$\eta_l(m) \sim \mathcal{N}(0,\sigma_n^2)$ is the AWGN,
and $\omega_j(m)$
is the $m$-th entry of $\{ \pmb{\omega}_j\in\mathbb{C}^M \mid \forall j\in\mathcal{T} \}$.

In order to average out the random phases
and obtain a real output, 
the euclidean norm of $\pmb{r}_l$ is taken, 
which leads to the expression,
\begin{equation}
	\label{eq:recv_norm}
	\begin{aligned}
	\lVert \pmb{r}_l \rVert^2 &= M \sum_{j=1}^N \mu_j^2 |\xi_{jl}|^2 + \underbrace{\sum_{j=1}^N \sum_{\substack{p=1\\ p\neq j}}^N \mu_j \mu_p \xi_j \xi_p^* \Big( \sum_{m=1}^M \nu_{jm} \nu_{pm}^* \Big)}_{\Delta_1} \\
	&+ \underbrace{2\sum_{j=1}^N \mu_j \Re\Big(\xi_j \sum_{m=1}^M \eta_{lm}^* \nu_{jm} \Big)}_{\Delta_2} + \underbrace{\sum_{m=1}^M |\eta_{lm}|^2}_{\Delta_3}.
	\end{aligned}
\end{equation}

The first term contains 
the desired output.
The terms 
$\Delta_{1}$,
$\Delta_{2}$,
and
$\Delta_{3}$ 
represent
the noise. 
The following lemma analyzes 
the statistics of the noise terms.

%We apply the operator $\Gamma(\pmb{r}_l) = \frac{1}{M}\lVert\pmb{r}_l\rVert^2 - \sigma_n^2$ on the received vector to obtain a desired transformation given by the following lemma.

\begin{lemma}
\label{lemma:delta}
Given a realization $\pmb{\mu} = \{\mu_j\ |\ \forall j\in \mathcal{T}\}$, the mean and variance of the noise term $\Delta = \frac{1}{M} (\Delta_1 + \Delta_2 + \Delta_3)$ are given by $\mathbb{E}\{\Delta | \pmb{\mu}\} = \sigma_n^2$ and
\begin{equation}
	\footnotesize
	\label{eq:delta_stats}
	\begin{aligned}
	\mathrm{Var}\{\Delta | \pmb{\mu}\} &= 2 \sum_{j=1}^N \sum_{\substack{p=1 \\ p>j}}^N \mu_j^2 \mu_p^2 (\sigma_{\xi_j}^2 - \bar{\xi}_j^2) (\sigma_{\xi_p}^2 - \bar{\xi}_p^2)\\ 
	&+ 2 \sigma_n^2 \sum_{j=1}^N \mu_j^2 (\sigma_{\xi_j}^2 - \bar{\xi}_j^2) + \sigma_n^4
	\end{aligned}
\end{equation}
where $\bar{\xi}_j$ and $\sigma_{\xi_j}^2$ denotes the mean and variance of random variable $\xi_j$, respectively.
\begin{proof}
	The proof follows from the discussions in \cite[p.87-94]{goldenbaum2014computation}.
	%\subsection{Analysis of additive noise term $\Delta_l$ in eq. \ref{eq:receiver_output}}
	%\label{AP:1}
	%We present an analysis of statistics (asymptotic and approximate) of overall noise $\Delta = \Delta_l$ in equation \ref{eq:receiver_output}. First we provide statistical analysis of independent terms in $\Delta$, and then provide analysis of cross-correlations of these terms.
	%
	%Starting with the term $\Delta_1$,
	%\begin{equation}
	%\begin{aligned}
	%	\Delta_1 &= \frac{1}{M} \sum_{j=1}^{|N_l|} \sum_{p=1, p\neq j}^{|N_l|} \xi_{jl} \xi_{jp}^* \ \sqrt{\mu_j \mu_p}\ \sum_{m=1}^{M} \nu_j(m) \nu_p^*(m) \\
	%	&= \frac{2}{M} \sum_{n=1}^N \tilde{\xi}_n \sqrt{\tilde{\mu}_n} \sum_{m=1}^{M} \cos(\theta_n(m)),
	%\end{aligned}
	%\end{equation}
	%where $N := |N_l|(|N_l|-1) / 2$, $\tilde{\xi}_n := \xi_{jl} \xi_{jp}^*$, $\tilde{\mu}_n := \mu_j \mu_p$, and $\theta_n(m) := (\theta_j(m) - \theta_p(m)) \, \text{mod} \, 2\pi $. The mapping $(j,p) \mapsto n$ is obtained by $n = n(j,p) = p + (j-1)|N_l| - j(j+1)/2,\ j=1,\dots,|N_l|,\ p=1,\dots,|N_l|$.
	%
	%Statistics of $\varepsilon = \cos(\theta_n)$, for $\theta_n$ uniformly distributed in $[0,2\pi)$ is given by
	%\begin{equation*}
	%p_{\varepsilon}(\varepsilon) = \frac{1}{\pi\sqrt{1-\varepsilon^2}} \mathrm{1}_{(-1,1)}(\varepsilon),\ \mathbb{E}\{\varepsilon\} = 0,\	\mathrm{Var}\{\varepsilon\} = \frac{1}{2}
	%\end{equation*}
	%
	%\begin{equation}
	%\mathbb{E}\{\Delta_1\} = \frac{2}{M}\sum_{n=1}^N \mathbb{E}\{ \tilde{\xi}_n\} \mathbb{E}\{\sqrt{\tilde{\mu}_n}\} \sum_{m=1}^{M} \mathbb{E}\{\cos(\theta_n(m))\} = 0,
	%\end{equation}
	%since expectations of both $cos(\theta_n(m))$ and $\tilde{\xi}_n := \xi_{jl} \xi_{pl}^*\ , j\neq p$ random variables are zero.
	%
	%Variance of $\Delta_1$ is given by
	%
	%\begin{equation}
	%\begin{aligned}
	%\mathrm{Var}\{\Delta_1\} &= \frac{4}{M} \sum_{n=1}^N \Big[ \mathbb{E}\{\tilde{\xi}_n \tilde{\xi}_n^*\}\ \mathbb{E}\{ \tilde{\mu}_n\}\ \sum_{m=1}^M\Big(\mathrm{Var}\{ \cos(\theta_n(m))\} \Big) \Big]\\
	%&= 2 \sigma_\xi^4 \sum_{n=1}^N \mathbb{E}\{\tilde{\mu}_n\}
	%\end{aligned}
	%\end{equation}
	%
	%As for the second term $\Delta_2$,
	%\begin{equation}
	%\begin{aligned}
	%\Delta_2 &= \frac{2}{M} \sum_{k=1}^{|N_i|} \sqrt{P_k}\ \Re\{h_{ik}\ \mathbf{S}_k\ \mathbf{n}^H_i\}\\
	%&= \frac{2}{M} \sum_{k=1}^{|N_i|} \sqrt{P_k}\, \\ & \Big[\Re\{h_{ik}\} \sum_{m=1}^M (\cos(\phi_k[m]) \Re\{n[m]\} + \sin(\phi_k[m]) \Im\{n[m]\})\\ & - \ \Im\{h_{ik}\} \sum_{m=1}^M (\sin(\phi_k[m]) \Re\{n[m]\} - \cos(\phi_k[m]) \Im\{n[m]\}) \Big].
	%\end{aligned}
	%\end{equation}
	%% where $\phi = (\phi_h + \phi_k[m] - \phi_n[m]) \, \text{mod}\, 2\pi$ is uniformly distributed in $[0, 2\pi)$, $\mathbb{E}\{\cos(\phi)\} = 0$, and hence $\mathbb{E}\{\Delta_2\} = 0$.
	%
	%Expectation of real and imaginary part of both noise and fading coefficients is zero. Moreover, fading coefficients, noise and phase of transmitted signals are independently distributed. These observations leads to following statistics of $\Delta_2$,
	%
	%\begin{equation}
	%\begin{aligned}
	%\mathbb{E}\{\Delta_2\} &= 0,\\
	%\mathrm{Var}\{\Delta_2\} &= 2 \sigma_h^2 \sigma_n^2 \sum_{k=1}^{|N_i|} \mathbb{E}\{P_k\}
	%\end{aligned}
	%\end{equation}
	%
	%Lastly, $\Delta_3 = \frac{1}{M} \sum_{m=1}^M n_i[m] n_i^*[m]$ is chi-squared distributed $\chi^2(2M)$
	%\begin{equation}
	%\begin{aligned}
	%\mathbb{E}\{\Delta_3\} &= \sigma_n^2 \\
	%\mathrm{Var}\{\Delta_3\} &= \sigma_n^4
	%\end{aligned}
	%\end{equation}
	%
	%Cross-correlation terms, $\mathbb{E}\{\Delta_i \Delta_j\},\ i,j=\{1,2,3\},\ i\neq j$, are mutually independent, since	$\mathbb{E}\{\Delta_i \Delta_j\} \propto \mathbb{E}\{n_k\} = 0 $.
	%
	%Hence, the complete second order statistics of $\Delta$ is given by
	%\begin{equation}
	%\begin{aligned}
	%\mathbb{E}\{\Delta\} &= \sigma_n^2 \\
	%\mathrm{Var}\{\Delta\} &= 2\sigma_h^4 \sum_{k=1}^{|N_i|} \sum_{l=1,\,l>k}^{|N_i|} \mathbb{E}\{P_k P_l\} \\ &+ \ 2\sigma_h^2 \sigma_n^2 \sum_{k=1}^{|N_i|} \mathbb{E}\{P_k\} \ + \ \sigma_n^4 
	%\end{aligned}
	%\end{equation}
	%
	%Without any apriori knowledge of each agents transmit values we cannot further simplify the expression for distribution of $\Delta$. Henceforth, we calculate the conditional distribution of $\Delta$, conditioned on a realization of transmit values of each agent given by $\mathbf{p}$. Assume that $\mathbb{E}\{P_k\} = p_k$ and $\mathbb{E}\{P_k P_l\} = \sigma_{p_{kl}},\ k \neq l$. Variance of $\Delta$ conditioned on realization $\mathbf{p}$ is given by
	%
	%\begin{equation}
	%\begin{aligned}
	%\sigma_{\Delta} = \mathrm{Var}\{\Delta | \mathbf{p}\} &= 2\sigma_h^4 \sum_{k=1}^{|N_i|} \sum_{l=1,\,l>k}^{|N_i|} \sigma_{p_{kl}} \\ &+ \ 2\sigma_h^2 \sigma_n^2 \sum_{k=1}^{|N_i|} p_k \ + \ \sigma_n^4
	%\end{aligned}
	%\end{equation}
	%
	%As the number of terms summing up to $\Delta$ are relatively large ($|N_i|(|N_i|-1)M/2 + 2|N_i|M + 2M$), we can invoke Central Limit Theorem to approximate the conditional distribution by a normal distribution.
	%
	%\begin{equation}
	%p(\Delta|\mathbf{p}) \rightarrow \mathcal{N}(\sigma_n^2, \sigma_{\Delta})
	%\end{equation}
\end{proof}
\end{lemma}
In accordance with \cite[prop. 5.2]{goldenbaum2014computation}, 
we can approximate the distribution of $\Delta|\pmb{\mu}$ as a normal distribution 
(for sufficiently large values of $M$ and $N$)
with mean and variance given by Lemma \ref{lemma:delta}.
\begin{assumption}
\label{as:noise}
In practical systems operating on high SNR regime, both $\xi_j\ \forall j \in \mathcal{T}$ and $\eta_l$ are sufficiently smaller than the desired output $\sum_{j=1}^N \mu_j^2 |\xi_j|^2$ for any given realization of $\pmb{\mu}$, such that the random variable $\tilde{\Delta} = \Delta - \sigma_n^2$ approaches zero asymptotically with $M$ and $N$.
\end{assumption}

In what follows, we assume that the noise term is equal to its expected value, 
i.e. $\Delta \equiv \sigma_n^2$. 
The following operator $\Gamma:\mathbb{C}^M\mapsto\mathbb{R}$ transforms the received signal
to obtain the desired signal, with vanishing noise asymptotically:
\begin{equation}
	\label{eq:opGamma}
	\forall \pmb{r}\in\mathbb{C}^M,\ 
	\Gamma(\pmb{r}) := \frac{1}{M}\lVert \pmb{r}\rVert^2 - \sigma_n^2 .
\end{equation}

The second orthogonal signal $\pmb{r}'_l$ is transformed using the same operator $\Gamma$ to obtain, 
\begin{equation}
\label{eq:gamma'}
	\gamma'_l :=\Gamma(\pmb{r}_l')= \frac{1}{M} \lVert \pmb{r}'_l \rVert^2 - \sigma'^2_n = \sum_{q=1}^N |\xi_{ql}|^2 .
\end{equation}
% where mean and variance of $\tilde{\Delta}'$ is obtained using $\forall j \in \mathcal{T}, \mu_j = 1$ in Lemma \ref{lemma:delta}.

Furthermore, in order to remove the scaling effect introduced by $\Phi$ during transmission,
let the de-scaling function $\Psi:\mathrm{P}\mapsto \mathrm{S}$ be
\begin{equation}
	\label{eq:opPhi-1}
	\forall \pmb{r}\in\mathbb{C}^M,\ 
	\Psi(\pmb{r}, \gamma'):= \frac{1}{\alpha} (\pmb{r} - \beta \gamma'),
\end{equation}
where $\alpha = \frac{P_{\max} - P_{\min}}{K_{\max} - K_{\min}} \in \mathbb{R}_{>0}$, $\beta = P_{\min} - \alpha S_{\min}$, and $\gamma'$ is obtained from the orthogonal signal, as in equation (\ref{eq:gamma'}).

\begin{proposition}
	\label{prop:noiseNeglect}
	A receiver $l\in\mathcal{N}$ and
	a set of transmitters $\mathcal{T}$ are given.
	Given 
	$\pmb{r}_l$ as in (\ref{eq:rl}),
	the operator $\Gamma$ as in (\ref{eq:opGamma}),
	and
	the operator $\Psi$ as in (\ref{eq:opPhi-1}),
	let $\gamma_l\in \mathrm{S}$ be 
	$\gamma_l :=\Psi(\Gamma(\pmb{r}_l)))$.
	The following holds:
	\begin{equation}
	\label{eq:receiver_output}
		\gamma_l = \sum_{j=1}^N x_j |\xi_{jl}|^2 .
	\end{equation}
	% where $\frac{1}{\alpha} \tilde{\Delta} \rightarrow \mathcal{N}(0, \frac{1}{\alpha^2} \mathrm{Var}\{\Delta\})$ and the approximation on the right is due to Assumption \ref{as:noiseless}.
\begin{proof}
The proof follows directly from Lemma \ref{lemma:delta}, Assumption \ref{as:noise}, and definitions of operators $\Gamma$ and $\Psi$. % In equation (\ref{eq:receiver_output}), $\Delta_l = \Delta - \sigma_n^2$ with $\sigma_{\Delta_l} = \mathrm{Var}\{\Delta\}$. We also argue that the variance of $\Delta$ will be small as compared to the absolute value of $\sum_{j=1}^N \Phi(\kappa_j) |\xi_{jl}|^2$. This is due to the fact that variance of channel and noise are relatively small for high SNR regime.
\end{proof}
\end{proposition}
%By this latter result,
%it is possible to state a result
%also for the noise in (\ref{eq:gamma'}).
%\begin{corollary}	
%	Given $\gamma_l'$
%	as in (\ref{eq:gamma'}),
%	the following holds:
%	\begin{equation}
%		\label{eq:receiver_den_output}
%		\gamma_l' =  \sum_{j=1}^N |\xi_{jl}|^2 + \tilde{\Delta}'\approx\sum_{j=1}^N |\xi_{jl}|^2.
%	\end{equation}
%	\begin{proof}
%		As in Proposition \ref{prop:noiseNeglect},
%		due to Assumption \ref{as:noiseless},
%		$\tilde{\Delta}'$ can be neglected.
%	\end{proof}
%\end{corollary}
%
%\begin{remark}
%	Note that the noise $\frac{1}{\alpha} \tilde{\Delta}$ has zero mean and negligible variance for high SNR regime and large $\alpha$. However, for values of $\alpha$ close to zero, the noise will be significant, and cannot be ignored anymore.
%\end{remark}
%
%
%
%\begin{remark}
%	\label{rmk:distChC}
%	$\varsigma := \sum_{q=1}^N |\xi_{ql}|^2\ \sim \frac{\sigma_\xi^2}{2}\chi^2_{2N}$ is chi-square distributed with $\mathbb{E}\{\varsigma\} = N\sigma_\xi^2$ and $\mathrm{Var}\{\varsigma\} = N \sigma_\xi^4$. For relatively small values of $\sigma_\xi$ and $\sigma_n$, the variance of $\Delta'_l$ is significantly smaller than the value of $\varsigma$. Hence, it is reasonable to ignore the noise $\Delta'_l$ in $\gamma'_l$.
%\end{remark}

%Finally, an output is obtained 
%by computing
%\begin{equation}
%	\psi_l(\frac{\gamma_l}{\gamma'_l})
%\end{equation}
%
%dividing the scalar
%$\gamma_l$ 
%by the scalar $\gamma'_l$ 
%and by applying the post-processing function $\psi_l: \mathbb{R} \mapsto \mathrm{S}$.
%This allows to obtain a 
%nomographic representation 
%in the sense of
%(\ref{eq:nomo}). 
Finally, the input-output relationship of the overall communication system
is summarized in the following definition:

\begin{definition}[Analog WMAC communication scheme]
	\label{rmk:distChC}
	Figure \ref{fig:commsys} describes the proposed analog communication system between 
	some transmitters and a single receiver
	$l\in\mathcal{N}$. 
	Inputs to this system are 
	the information states
	at iteration $k\in\mathbb{N}$
	of transmitters in $N_l$,
	which are grouped in vector $\mathbf{x}_{N_l}(k) \in \mathrm{S}^{|{N}_l|}$. 
	The output is given by
	\begin{equation}
	\label{eq:WMAC_output}
		\hat{f}_l(\mathbf{x}_{N_l}(k)) = \frac{\gamma_l}{\gamma'_l} = \sum_{j\in {N}_l}h_{lj}(k)x_j(k) ,
	\end{equation}
	where, 
	$\forall j \in {N}_l,\ \forall k\in\mathbb{N},\ h_{lj}(k) := \frac{|\xi_{jl}(k)|^2}{\sum_{q\in {N}_l} |\xi_{ql}(k)|^2}\ \in (0, 1]$ is the normalized channel fading coefficient.
	Clearly, by construction,
	$\forall l\in\mathcal{N},\ \forall k\in\mathbb{N},\ \sum_{j\in N_l}h_{lj}(k)=1$.
%	\begin{proof}
%	Since $\Phi$ simply applies scaling and shifting by scalar transformations, therefore its inverse $\Phi^{-1}$ exists. Now, consider
%	\begin{equation}
%		\begin{aligned}
%			\Phi^{-1} \frac{\gamma_l}{\gamma'_l} &= \Phi^{-1} \Big( \frac{\sum_{j=1}^N \Phi(\kappa_j) |\xi_{jl}|^2}{\sum_{p=1}^N |\xi_{pl}|^2} \Big) \\
%			&= \sum_{j=1}^N \Phi^{-1} \Phi(\kappa_j) \frac{|\xi_{jl}|^2}{\sum_{p=1}^N |\xi_{pl}|^2} = \sum_{j=1}^N \phi_j(x_j) h_{jl}
%		\end{aligned}
%	\end{equation}
%	where $\kappa_j = \phi_j(x_j)$ and $h_{jl} = \frac{|\xi_{jl}|^2}{\sum_{p=1}^N |\xi_{pl}|^2}$.
%	\end{proof}
\end{definition}
%\hl{
%Clearly, it will be possible
%to choose a family of pre-processing
%and post-processing functions,
%depending on the realizations 
%of the normalized channel fading coefficients,
%such that (\ref{eq:WMAC_output})
%can be used to compute 
%(\ref{eq:nomo}).
%}

The signal $\hat{f}$
has the desired characteristics
(see Section \ref{sec:wirelessMAC}).
An empirical analysis of probability distribution
of error between true $f$ and $\hat{f}$, as
presented in Appendix \ref{AP:error},
shows that the assumption \ref{as:noise} is valid.
In fact,
$\forall l\in\mathcal{N}$,
$\forall k\in\mathbb{N}$,
$$\hat{f}_l(\mathbf{x}_{N_l}(k))\in\mathcal{C}(\{ x_j(k) \mid j\in N_l \})\subset\mathbb{R}.$$
The presented communication
system will
be employed
by the consensus protocol
presented in the next section.


==> keywords.tex <==
% Note that keywords are not normally used for peerreview papers.
\begin{IEEEkeywords}
Consensus, Wireless, Multi-Agent, Cooperative Control.
\end{IEEEkeywords}

==> noise_quantization.tex <==
\section{Benefits of this approach}
\subsection{Converging time}
Fabio
\subsection{Battery life}
Navneet

==> nomographic_approach.tex <==
\section{{Nomographic representations of \textit{MAX}}}
Two nomographic representations of 
$\max: \mathrm{S}^N \mapsto \mathrm{S}$ are here presented, 
where $ \mathrm{S} \subset \mathbb{R} $ is a compact set. 
According to Theorem \ref{thm1}, there exist at least $N\times (2N+1)$ continuous univariate pre- and post-processing functions that can form a nomographic representation of $\max$. However, there is no constructive method for finding these functions in general. 
We propose the two following nomographic approximation 
of max-function and analyze their performance by implementing them using the communication system described in the previous section. 

%Table \ref{tab:operations} lists respective operations corresponding to the approximate max-function computation over WMAC.
%
%%We assume, without loss of generality, that the maximum transmit power of each agent is $P_{\max} = 1$, and information states $s_k[t]$ are taken from a real and compact set, $\mathrm{S} = [0,1]$. 
%
%
%
%
%\begin{table}[!thb]
%	\begin{center}
%		% \renewcommand{\arraystretch}{1.2}
%		\begin{tabular}{|>{$}m{0.1\columnwidth}<{$}|>{$}m{0.175\columnwidth}<{$}|>{$}m{0.175\columnwidth}<{$}|>{$}m{0.175\columnwidth}<{$}|>{$}m{0.175\columnwidth}<{$}|}
%			\hline \\
%			 \hat{f}_{\max}	& \multicolumn{2}{|c|}{\textbf{Sum-of-powers}} 	& \multicolumn{2}{|c|}{\textbf{Log-sum-exp}} \\
%			\hline \\
%			 	& \text{expr}	& \text{range} 	& \text{expr}	& \text{range} \\
%			\hline \\
%			x_j			& x		& [0,1]		& x 	& [0,1]\\
%			\hline \\
%			\phi_j(\cdot) 			& x^p 	& [0,1]		& \exp(x \cdot p)	& [1, \exp(p)]\\
%			\hline \\
%			\mathcal{F}(\cdot) 		& x^p * (\sqrt{P_{\max}} - \sqrt{P_{\min}})  + \sqrt{P_{\min}}	& [\sqrt{P_{\min}}, \sqrt{P_{\max}}]	& \frac{\exp(x p) - 1}{\exp(p) - 1} * (\sqrt{P_{\max}} - \sqrt{P_{\min}})  + \sqrt{P_{\min}}	& [\sqrt{P_{\min}}, \sqrt{P_{\max}}] \\
%			\hline \\
%			\mathcal{G}(\cdot) 		& \xi 								& (\exp(p) - 1)\ x \\
%			\hline \\
%			%\mathcal{D} 	& \frac{1}{M} (x - \mu_z) 			& \frac{1}{M} (x - \mu_z) \\
%			%\hline \\
%			\psi_i(\cdot) 			& \sqrt[p]{x} 						& \frac{1}{p} \ln(x) + 1 \\
%			%\hline \\
%			%\hat{f}_{\max}(\mathbf{s}[t]) & \Big( \sum_{k \in N_i} H_{ik}\ (s_k[t])^p \Big)^{\frac{1}{p}} & \frac{1}{p}\ \ln\Big( \sum_{k \in N_i} H_{ik}\ \frac{e^{s_k[t] \cdot p} - 1}{e^p - 1} \Big) + 1 \\
%			\hline
%		\end{tabular}
%	\end{center}
%	\caption{Operations for function computation over WMAC }
%	\label{tab:operations}
%\end{table}


\begin{definition}[Sum-of-powers]
	\begin{equation}
	\hat{f}^s_{\max}(\{x_1, \dots, x_N\}, p) = \Big( \sum_{j=1}^N \alpha_j x_j^p \Big)^{1/p},
	\end{equation}
	where $\alpha_j \geq 0$. %Pre- and post-processing function defined as $\phi_k^s(x) = x^p$ and $\psi_i^s(x) = x^{\frac{1}{p}}$, respectively.
\end{definition}

\begin{corollary}
	\begin{equation}
	\hat{f}^s_{\max}(\{x_1, \dots, x_N\}, p) = \max(x_1, \dots, x_N) + \epsilon
	\end{equation}
	where $|\epsilon| \rightarrow 0$ as $p \rightarrow \infty$.
	\begin{proof}
		Assuming that the inputs $\{x_1, \dots, x_N\}$ are sorted with $x_1 \geq x_2 \geq \dots \geq x_N$.
		\begin{equation*}
		\hat{f}^s_{\max}(\{x_1, \dots, x_N\}, p) =  x_1\ \Big( \sum_{j=1}^N \alpha_j\ \big(\frac{x_j}{x_1}\big)^p \Big)^{\frac{1}{p}}
		\end{equation*}
		Given that $0 < \alpha_j \leq 1$ and $x_j \in \mathcal{S},\ \forall j$, we have $\sum_{j=1}^N \alpha_j \big(\frac{x_j}{x_1}\big)^p \leq \sum_{j=1}^N \alpha_j < N$ due to the fact that $\big(\frac{x_j}{x_1}\big)^p \leq 1$. For $N \geq 1$, $ N^{1/p} \xrightarrow[]{p \rightarrow \infty} 1$, and hence $\hat{f}^s_{\max}(x_1, \dots, x_N) \xrightarrow[]{p \rightarrow \infty}  x_1 = \max(x_1, \dots, x_N)$.	
	\end{proof}
\end{corollary}

\begin{definition}[Log-sum-exp]
	\begin{equation}
	\hat{f}^l_{\max}(x_1, \dots, x_N) = \frac{1}{p} \ln \Big( \sum_{j=1}^N \alpha_j \exp(x_j\ p) \Big).
	\end{equation}
	where $\alpha_j \geq 0$. %Pre- and post-processing function defined as $\phi_k^l(x) = \exp(x \cdot p)$ and $\psi_i^l(x) = \frac{1}{p} \ln(x)$, respectively.
\end{definition}

\begin{corollary}
	\begin{equation}
	\hat{f}^l_{\max}(x_1, \dots, x_N) =  \max(x_1, \dots, x_N) + \epsilon
	\end{equation}
	where $|\epsilon| \rightarrow 0$ as $p \rightarrow \infty$.
	\begin{proof}
		\begin{equation*}
		\hat{f}^l_{\max}(\{x_1, \dots, x_N\}, p) =  x_1 + \lim_{p \rightarrow \infty} \ln\Big( \sum_{j=1}^N \alpha_j e^{(x_j - x_1)\,p} \Big)^{1/p}
		\end{equation*}
		Since $x_1 - x_j \geq 0$, we have $\sum_{j=1}^N \alpha_j e^{-(x_1 - x_j)p} \leq \sum_{j=1}^N \alpha_j \leq N$. Therefore, the term $ \lim_{p \rightarrow \infty} \Big( \sum_{j=1}^N \alpha_j e^{(x_j - x_1)\,p} \Big)^{1/p} \rightarrow 1$, and hence $\hat{f}^l_{\max}(\{x_1, \dots, x_N\}, p) \xrightarrow[]{p \rightarrow \infty} x_1 = \max(x_1,\dots,x_N)$.
	\end{proof}
\end{corollary}

\begin{figure}[!hbt]
	\centering
	\includegraphics[width=.5\columnwidth]{fig/nom_fig}
	\caption{Nomographic approximations of $\max$ function. \hl{shrink}}
	\label{fig:nomo}
\end{figure}

%A large value of $M$ will make the contribution of $x_{\max} = \max(x_1, \dots, x_N)$ exponentially more that contributions from other values. Then the $\frac{1}{M}\ln$ function will convert the exponential back to its original value. 

%\subsection{Max-consensus in WMAC via nomographic approximations}
%In this section we analyze the performance of the approximate nomographic functions $\hat{f}_{\max}$ described above, using the analog computation over WMAC approach described in section \ref{A-WMAC}. Accordingly, each agent $k \in N_i$ will transmit pre-processed information given by $\phi_k^s(x_k) = x_k^p$ or $\phi_k^l(x_k) = \frac{e^{Mx_k} - 1}{e^M - 1}$, and the receiver of agent $i$ will apply respective post-processing functions to the signal received from its $|N_i|$ neighbors, given by $ \psi^s(x) = x^{1/p}$ or $\psi^l(x) = \frac{1}{M} \ln (x) + 1$.
%
%According to equation (\ref{eq:awmac}), the received value at the receiving agent $i$ using \textit{sum of powers} max-function approximation, is given by
%
%\begin{equation}
%\begin{aligned}
%s_i^s(t) &= \Big( \sum_{k=1}^{|N_i|} H_{ik}(t)\ P_k(t)^p \Big)^{1/p}\\
%&= \Big( H_{im}(t)\ P_m(t)^p + \sum_{k=1, k\neq m}^{|N_i|} H_{ik}(t)\ P_k(t)^p \Big)^{1/p}\\
%&= \underbrace{H_{im}^{1/p}(t)}_{\sim 1}\ P_m(t) \underbrace{\Big(1 + \sum_{k=1, k\neq m}^{|N_i|} \frac{H_{ik}(t)}{H_{im}(t)}\ \Big(\frac{P_k(t)}{P_m(t)}\Big)^p \Big)^{1/p}}_{\sim 1}\\
%&\sim P_m(t)
%\end{aligned}
%\end{equation}
%where $m$ is the index for maximum value term, and approximations are valid for $p \gg |N_i|$.
%
%Similarly, the received value at the agent $i$ using \textit{log-sum-exp} max-function approximation, is given by
%\begin{equation}
%\begin{aligned}
%s_i^l(t) =\ &\frac{1}{M} \ln\Big( \sum_{k=1}^{|N_i|} H_{ik}(t)\ \frac{e^{M P_k(t)} - 1}{e^M - 1} \Big) + 1\\
%=\ &\frac{1}{M} \ln\Big(  \sum_{k=1}^{|N_i|} H_{ik}(t)\ (e^{M P_k(t)} - 1) \Big) - \underbrace{\Big(\frac{1}{M} \ln (e^{M} - 1) \Big) + 1}_{\sim 0}\\
%\sim\ &\frac{1}{M} \ln\Big( H_{im}(t) e^{MP_k(t)} + \sum_{k=1, k\neq m}^{|N_i|} H_{ik}(t)\ (e^{M P_k(t)} - 1) \Big)\\
%\sim\ &P_m(t) + \Delta_l\\
%\Delta_l =\	&\frac{1}{M} \ln (H_{im}(t)) + \frac{1}{M} \ln \Big( 1 + \sum_{k=1, k\neq m}^{|N_i|} \frac{H_{ik}(t)}{H_{im}(t)}\ \frac{e^{M P_k(t)}}{e^{M P_m(t)}} \\
%& \qquad \qquad - \sum_{k=1, k\neq m}^{|N_i|} \frac{H_{ik}(t)}{H_{im}(t)e^{M P_m(t)}} \Big) \sim 0\\
%\Delta_l \sim\ &0 \Rightarrow  s_i^l(t) = P_m(t)
%\end{aligned}
%\end{equation}
%for $M \gg |N_i|$. Hence, we have proved that for $p,M \gg |N_i|$ both nomographic functions approximate to the max-function. 

% However, this is only valid when SNR of the transmitted signal is high for at least the max valued agent. Since, the transmit signal power is proportional to the state of the agent, we cannot guarantee that SNR will be high for the max agent. For example, if the max of all the neighboring agents of agent $i$ have state value close to $0$, the transmitted signal power will be close to $0$ as well, and hence the SNR of even the maximum power signal will be very low. In that case, the noise will dominate all the received signals and the equation (\ref{A-WMAC}) will not give a good approximation of weighted sums of transmitted signals. Therefore, in what follows, we present a novel strategy for max-consensus in WMAC which is independent of distribution of the states of agents.

\begin{remark}
As shown in Figure \ref{fig:nomo}, both approximations of max approaches close to the true max as value of $p$ tends to infinity. However, for practical communication system with finite value of $p$, the value of scaling coefficient $\alpha$, as described in Section \ref{sec:commsys}, will tend to zero as $p$ tends to infinity. This will lead to high noise levels in the output of the receiver, leading to high approximation error $|\epsilon|$. A positive error $\epsilon$ at some time instant $k$ in the iteration will shift the initial maximum value to a new maximum. This will lead to failure of max consensus iterative algorithm, as described in equation (\ref{eq:necessaryForMax}). Hence, the nomographic approximations of $\max$ presented in this section, will fail for communication system described in Section \ref{sec:commsys}.
\end{remark}

